On the Effectiveness of Machine Learning-based Call Graph Pruning: An Empirical Study

Static call graph (CG) construction often over-approximates call relations, leading to sound, but imprecise results. Recent research has explored machine learning (ML)-based CG pruning as a means to enhance precision by eliminating false edges. However, current methods suffer from a limited evaluation dataset, imbalanced training data, and reduced recall, which affects practical downstream analyses. Prior results were also not compared with advanced static CG construction techniques yet. This study tackles these issues. We introduce the NYXCorpus, a dataset of real-world Java programs with high test coverage and we collect traces from test executions and build a ground truth of dynamic CGs. We leverage these CGs to explore conservative pruning strategies during the training and inference of ML-based CG pruners. We conduct a comparative analysis of static CGs generated using zero control flow analysis (0-CFA) and those produced by a context-sensitive 1-CFA algorithm, evaluating both with and without pruning. We find that CG pruning is a difficult task for real-world Java projects and substantial improvements in the CG precision (+25%) meet reduced recall (-9%). However, our experiments show promising results: even when we favor recall over precision by using an F2 metric in our experiments, we can show that pruned CGs have comparable quality to a context-sensitive 1-CFA analysis while being computationally less demanding. Resulting CGs are much smaller (69%), and substantially faster (3.5x speed-up), with virtually unchanged results in our downstream analysis.

==> sections/abstract.tex <==
% !TEX root = ../main.tex

\todo{this is WAY to long for an abstract: 1) shorten to about 1/3 of a text column 2) add everything to a single paragraph (if you need a second one for structuring, you know that it is to long). Focus on (a) what is the context and the problem? Why is research here necessary? touch(!) upon the shortcomings of previous work (b) What is your idea for improvement? (c) touch(!) upon you methodology (d) touch(!) upon you results}

\todo{Avoid using concrete tool names of other tools in the abstract... for the rest of the paper write \tool{CGPruner} instead of CGPruner (Write Latex like HTML and prefer semantic formatting commands over basic macros like defining a \textbackslash{}cgpruner command)}

Static call graph construction tends to over-approximate call relations, which leads to poor precision. To address this, scholars have recently proposed machine learning (ML)-powered call graph pruning to eliminate false edges and improve the precision of call graphs. CGPruner and AutoPruner are two existing ML-based call graph pruning models based on RandomForest and CodeBERT, respectively. The former uses structural features, while the latter uses combined features, i.e., structural and semantic features. Even though prior research shows promising results, they have three limitations: (1) Both research works have been trained and evaluated on a dataset with a relatively low branch coverage of 68\%. (2) Due to the over-approximation of static analysis, the dataset for learning a call graph pruner is quite imbalanced. (3) It is still unclear what the effect of using a minimalistic code context is on the call graph pruning when source code is unavailable for some call graph nodes.
This paper empirically studies the effectiveness of ML-based call graph pruning. Specifically, our research methodology addresses the mentioned issues by (1) considering two additional datasets in the evaluation, which contain real-world Java programs and 88\% branch coverage. (2) attempting to repair the prior work's dataset with complete source code for call graph nodes by using a de-compiler and finding source code repositories. (3) Integrating pruning goals into the training phase of call graph pruners to enable control over recall and precision.

In summary, our empirical findings show that, first, ML-based call graph pruning is effective on all three datasets, including real-world Java projects, and it significantly improves the precision of static call graphs. Second, de-compilation is promising to repair a dataset with source code as it gives comparable performance compared to the models trained on the original dataset. Third, integrating pruning goals into the learning phase can further boost the performance of call graph pruners. Finally, ML-based call graph pruning was shown to be computationally inexpensive compared to static call graph construction, and hence it can be used in practice.

==> sections/discussion.tex <==
% !TEX root = ../main.tex
\section{Discussion}
\label{sec:discuss}

\revise{Points to be discussed:
- Pre-trained models might have seen the target projects before, but this is not an issue as pre-training does not know anything about CGs or edge pruning.
- Test coverage is only the first step, as it is biased towards the target project. A 88\% coverage of the test projects translates to a much smaller coverage of the whol edependency set. Future work needs to look into collecting better datasets.
- contradiction to previous work regarding X(?) needs further research
}


When reflecting on the results of our previous experiments, we believe that several points are noteworthy for everyone working in this area and which should be considered in future research.

\todo{1) The discussion is not just a collection of findings... make sure that all points that you raise here go beyond just restating the observations of the paper. 2) Connect every point to an idea of future research! 3) do not use a simple list, flesh out the parts and use named paragraphs}

%%%%%%%%%%%
\paragraph{Call graph pruning is an open problem} Generally, code language models like CodeBert and CodeT5 substantially improve the precision of static call graphs, as shown in RQ1. However, we believe that the call graph pruning task is still challenging, especially for real-world programs. For such programs, we observed that it is more difficult for the models to retain true edges while pruning the false ones. Therefore, there is still room for improvement in future work in which scholars can explore more powerful models for the call graph pruning task.
\todo{this is a weak point as it is very unconcrete}

%\todo{so, what is your recommendation? word of caution to future tools/evaluations in this area?}

%%%%%%%%%%%
\paragraph{There are alternatives to complete source code for CG nodes} In RQ1.1, we found that the ML models have almost the same performance on all three versions of the NJR1 dataset: original, de-compiled, and recovered. This is different from our initial expectation. We initially thought recovering the dataset with complete source code would significantly improve the performance. However, our findings in RQ1.1 has also interesting implications for the ML-based call graph pruning task. In the absence of source code, using a de-compiler code can be promising, or one can still use a mix of semantic and signature-based features if not all call graph nodes have source code.
\todo{what is the wider reaching consequence here? More work on finding the best representation is needed? Or to find better features in general? What is the actionable insight here? As of now, the paragraph does not add anything on top of what has been said before and could safely be deleted}

%%%%%%%%%%%
\paragraph{The use of pruning goals is encouraged} Datasets for learning CG pruning are highly imbalanced (see P/R ratio in Table~\ref{tab:data-stats}). Hence, the trained ML models have a higher tendency to prune edges rather than retain them.
This results in a big loss in soundness or recall, i.e., losing true edges in call graphs.
With the introduction of pruning goals in RQ2, we found that the conservative pruning goal improves the pruned call graphs produced by the models, compared to no pruning goal at all. Given this finding, we suggest using a pruning goal when training a model.
Depending on the downstream analyses and trade-offs between recall and precision, one can choose balanced or conservative goals. Also, we advise against using the aggressive pruning goal as it greatly reduces the recall, even though it can make a call graph much smaller on the disk. 
\todo{If this is our main finding, why did we not experiment with an F2-measures to put more focus on recall?}

%%%%%%%%%%%
\paragraph{semantic feature is a viable choice} Different from the finding of the previous work~\cite{le2022autopruner}, our finding in RQ3 shows that the models trained with the combined feature set, the semantic and structural features together, give pruned call graphs with almost the same quality as the models trained only using the semantic feature. We attribute this to the fact that structural features, $f_{struct}$, are dominated by the semantic feature, $f_{sem}$, in the learning phase. Note that $f_{sem}$ has 768 elements whereas $f_{struct}$ has 11 features. Overall, we recommend using the semantic features for training CLM-based pruners as it provides a fair balance between acceptable performance and computational time.
\todo{can we envision any future work that is related to this? As is, the point is very weak, as it is mainly restating what has been said before.}

%%%%%%%%%%%
\paragraph{ML-based CG pruning is computationally inexpensive} The CG pruning task adds additional computational cost to the static call graph construction, which ranges from negligible cost for using small and fast models like \tool{CGPruner}~\cite{utture2022striking} to more substantial like in our case \tool{CodeBert}, which has much better results at the expense \textasciitilde 23\% computational overhead for feature extraction and model inference.
Overall, we believe that, despite the additional overhead, the use of ML-based call graph pruners can be justified given the significant improvement in the precision of call graphs. To further reduce the computational cost, it is possible to parallelize the extraction of structural features or use a more optimized tokenizer for extracting semantic features. Additionally, model inference can be sped up using an accelerator such as ONNX Runtime~\cite{onnx}.
\todo{As a general pattern in the discussion there is too much repetition going on and WAY too little pointing forwards. There are always multiple sentences repeating our findigns and one sentence that envisions future work. The ratio should be the other way around... summarize/repeat the findings in one sentence and then talk about stuff that has not been said before.}






==> sections/introduction.tex <==
% !TEX root = ../main.tex
\section{Introduction}
Call graphs (CG) represent function invocations within programs~\cite{ryder1979constructing, callahan1990constructing}.
Their construction is a crucial component of static program analysis, like security analysis, dead code identification, performance profiling, and more.
An ideal CG would be both \emph{sound}, i.e., not missing any legitimate function call, and \emph{precise}, i.e., not containing unnecessary function calls.
However, constructing a sound and precise CG is challenging even for small programs~\cite{ali2012application}.
In practice, static CG construction will over-approximate the call relations to boost soundness in favor of precision: popular tools like \tool{WALA}~\cite{fink2012wala} or \tool{Petablox}~\cite{mangal2015user} create imprecise CGs with up to 76\% false edges~\cite{utture2022striking}.
%A balanced approach between soundness and precision should be taken in call graph analysis.
To address this imprecision, previous work~\cite{bravenboer2009strictly, mangal2015user, tan2016making} have enhanced pointer analysis, which builds the backbone of numerous GC construction algorithms, by improving the context-sensitivity or flow-sensitivity.
Unfortunately, a flawless pointer analysis is generally infeasible~\cite{rice1953classes}, and pointer analyses often require a tradeoff between scalability and precision~\cite{li2018scalability}.
For instance, \tool{WALA}'s context-sensitive analysis only reduces the false positive rate by 8.6\% compared to a context-insensitive analysis, despite significantly slowing down performance~\cite{utture2022striking}.

Recent work has introduced Machine Learning (ML)-based call graph pruning approaches to improve the precision of call graphs by pruning false edges in call graphs as a post-processing step.
Tools like \tool{CGPruner}~\cite{utture2022striking} and \tool{AutoPruner}~\cite{le2022autopruner} learn from dynamic traces that are collected in actual program executions to identify unnecessary edges in a static CG.
\tool{CGPruner} only leverages features of the CG structure, while \tool{AutoPruner} combines structural features with automatically extracted semantic features from the source code that are encoded with the code language model, \tool{CodeBERT}~\cite{feng2020codebert}.
Although these previous approaches show intriguing results, they suffer from three limitations:
%
(1) Both have been trained and evaluated on the NJR-1 dataset~\cite{palsberg2018njr}, which suffers from a notoriously low branch coverage of 68\%.
This presents a severe threat to validity.
%
(2)
The over-approximation of static call graph construction results in a large number of unnecessary edges~\cite{reif2021novel} and dynamic CGs will contain much fewer edges.
As a result, the training and evaluation of the ML models has to deal with a highly imbalanced dataset.
%
(3) \tool{AutoPruner} mixes two code representations before extracting semantic features.
Project internal methods use their full source code, while code from dependencies is only represented with minimalistic method signatures.
The effect of this mixed representation or whether one representation is superior to the other is still unclear.

In this paper, we will address these issues by
(1) introducing two additional datasets, namely, XCorpus~\cite{dietrich2017xcorpus} and YCorpus, in our evaluation. Both have
real-world Java programs. Also, we created YCorpus for this work, which has 88\% branch coverage on average in their tests and is therefore particularly suitable for the call graph pruning task.
(2) An attempt to recover source code for the dependencies of the programs in the NJR-1 dataset by finding source code repositories and using a de-compiler
to translate byte code to Java source code.
(3) introducing pruning goals which are integrated into the learning phase of call graph pruners by employing weights in the loss function.
This not only helps to deal with an imbalanced dataset but also allows to define pruning strategies (e.g., deciding between conservative or aggressive edge pruning).
These three improvements allow us to study the following research questions:

\begin{description}
%
\item[\RQ{1}] How do ML-based CG pruning models perform on the NJR-1, XCorpus, and YCorpus datasets?
%How do ML-based CG pruners perform on other corpora?
%
\item[\RQ{2}] How do the ML models perform on the NJR-1 dataset if it is "repaired"?
%
\item[\RQ{3}] How do different code features contribute to the performance of the ML-based call graph pruning models?
%How do different code features contribute to the performance of the ML-based CG pruners?
%
\item[\RQ{4}] How do the ML models perform at the call graph pruning task considering different pruning goals?
%How do the ML models perform at the call graph pruning task considering different pruning strategies?
%
\item[\RQ{5}]  Which overhead does ML-based call graph pruning add?
%Which overhead does ML-based call graph pruning add?
\end{description}

Our main results show that: (1) ML-based call graph pruning techniques are effective on all three corpora and can boost the precision of static CGs.
We also observe that CG pruning seems to be more difficult on real-world Java projects.
(2) in contrast to the finding of previous work~\cite{le2022autopruner}, we find comparable pruning performance when using either semantic features or a combined feature set that also includes structure.
(3) to repair the NJR-1 dataset, de-compilation to restore source code can be as effective as recovering the original source code, given that the ML models trained on both versions perform
quite similarly. (4) By integrating the pruning goals into the training of call
graph pruning models, it is possible to overcome the imbalanced
nature of the datasets for the call graph pruning
task. (5) our performance measurements show that ML-based call graph pruning can boost the precision of CG construction at a negligible computational cost.

\smallskip
\noindent
Overall, this paper makes the following main contributions.

\begin{itemize}
\item To the best of our knowledge, this paper is the first empirical study on the effectiveness of ML-based call graph pruning, which studies its current issues, proposes solutions and evaluates their effects.
\item We created a new benchmark dataset, YCorpus, for the call graph pruning task. It has 88\% test coverage on average.
\item We publicly share five trained ML models for call graph pruning and three datasets, NJR-1, XCorpus, and YCorpus, to foster future research.\footnote{\todo{Share an anonymous Zenodo link here -- for the *review*, it should not be Zenodo... an anonymized Dropbox link is easier to update for us and perfectly fine}}
\end{itemize}

%The rest of this paper is organized as follows. We describe related work in section~\ref{sec:related-work}. We explain our research methodology in section~\ref{sec:approach}. The evaluation setup for this study is described in section~\ref{sec:eval-setup}. We present the obtained empirical results in section~\ref{sec:eval}. We discuss the implications of the obtained results in section~\ref{sec:discuss}. Finally, we conclude our empirical study in section~\ref{sec:summary}.



==> sections/rq-code-features.tex <==
% !TEX root = ../main.tex
\subsection{\RQ{3}: The performance of the models with different code features}

\begin{table*}[!t]
\centering
\caption{Comparison of the models on NJR-1, XCorpus and YCorpus with different code features}
\label{tab:diff-code-feat}
\vspace{-6pt}
\small
\input{tables/comparison-code-features}
\end{table*}

In section~\ref{sec:feat}, we explained five code features/representations to train ML models for the call graph pruning task. Hence, for this RQ, we aim to find out how these code features, i.e., structural, signature, semantics, combined would impact the performance of the ML models. Essentially, we want to understand how these models perform if trained from the least available information, i.e., signature-based feature, $f_{sig}$ to the richest representation, combined, $f_{comb}$. Moreover, we evaluate whether our proposed code representation, call site-based ($f_{cs}$), can improve the performance of the ML-based call graph pruners.
 
\paragraph{Methodology} For RQ3, we train and evaluate ML-based call graph pruning models \todo{tuning of hyper parameters?}
on the NJR-1, XCorpus, and YCorpus datasets with five different code features, namely, semantic-based ($f_{sem}$), structural-based ($f_{struct}$), signature-based ($f_{sig}$), call-site based ($f_{cs}$), and combined ($f_{comb}$). Also, for this RQ, we do not use any pruning goals.

\paragraph{Results} Table~\ref{tab:diff-code-feat} shows the performance of the models on the NJR-1, XCorpus, and YCorpus datasets with five different code representations.
The table shows \todo{briefly introduce the different columns}
The results for $f_{struct}$ and $f_{sem}$ are borrowed from Table~\ref{tab:general-perf} for the sake of comparison with other code features. Starting with the signature-based feature, $f_{sig}$, we observe the performance of the models is reduced on both NJR-1 and XCorpus datasets. This is expected as $f_{sig}$ provides no code context other than the method/target signatures. However, for YCorpus, the models trained with $f_{sig}$ give higher quality pruned call graphs than that of the models trained with $f_{sem}$. In the case of CodeT5, it has a 7\% higher F1-score. This finding is both surprising and unexpected. We attribute this to the likelihood that code language models might have seen the source/target methods in the test programs of YCorpus in their pre-training code corpus.
\todo{As is, this sounds like a MASSIVE, reject-worthy limitation.}
Concerning the $f_{comb}$ feature, it does not generally bring significant improvement across all three datasets compared to $f_{sem}$. Also, AutoPruner~\cite{le2022autopruner} with the $f_{comb}$ feature has almost the same performance in all three datasets compared to CodeBert with the $f_{sem}$ representation.

Lastly, for the call site-based representation ($f_{cs}$), in general, we do not observe substantial improvement over $f_{sem}$ for the ML-based call graph pruners. However, CodeBert and CodeT5+ are the only models that gained a small performance improvement on XCorpus and NJR-1, respectively, compared to other code features. This is in line with our intuition that the call site-based feature could potentially improve the performance by only including relevant code context in the body of the source method.

==> sections/rq-general-performance.tex <==
% !TEX root = ../main.tex
\subsection{\RQ{1}: The general performance of the ML models at the call graph pruning task}

First, it is prominent to assess the overall performance of the ML models, described in section ~\ref{sec:models}, and their capacity in pruning static call graphs. This assessment provides insights into the models' abilities and a benchmark for subsequent experiments including our attempt to repair the NJR-1 dataset and exploring different pruning strategies.
 
\paragraph{Methodology} To address RQ1, we used three datasets, NJR-1, XCorpus, and YCorpus, which are described in~\ref{subsec:datasets}. Specifically, for the NJR-1 dataset, same as the prior work~\cite{utture2022striking}, we trained the models, described in section~\ref{sec:models}, on 100 programs and we evaluated them on 41 programs. For XCorpus, we trained the models on 12 programs and evaluated them on 4 programs. Also, for YCorpus, we trained and evaluated the models on 15 and 3 projects, respectively. To find the optimal hyper-parameters for the RandomForest model, similar to the work of Utture et al.~\cite{utture2022striking}, we performed 4-fold cross-validation with grid search. To assess the quality of pruned static call graphs by the ML models, we used the evaluation metrics described in section~\ref{sec:eval-setup}.


\paragraph{Results} Table~\ref{tab:general-perf} shows the general performance of the ML models including CGPruner~\cite{utture2022striking} and AutoPruner~\cite{le2022autopruner} on the NJR-1, XCorpus, and YCorpus datasets.
The table shows the \emph{Precision}, \emph{Recall}, and \emph{F1 score} when comparing the ground truth to the pruned CG.
Our results show that the precision of pruned CGs is significantly higher than Wala's static call graphs.
For instance, considering YCorpus, CodeT5's precision is 53\%, which is 31\% higher than that of Wala.
We also observe that code language models, i.e., CodeT5 and CodeBert, substantially outperform CGPruner (i.e., RandomForest) across all three datasets in terms of F1.
This is expected as code language models leverage semantic features like source code context and also RandomForest seems to be more susceptible to imbalanced datasets (see P/R ratios in Table~\ref{tab:data-stats}).
Both XCorpus and YCorpus contain popular real-world Java projects in contrast to NJR-1, which focused on automation over popularity when selecting Java projects.
It is interesting to note that the F1 score is lower in both corpora compared to NJR-1, which suggests that the pruning task gets more challenging for CGs of real-world applications.

\begin{table}[t]
\centering
\caption{Comparison of the models on the XCorpus, NJR-1, and YCorpus datasets}
\label{tab:general-perf}
\vspace{-6pt}
\footnotesize
\input{tables/comparison-all-datasets}
\end{table}


==> sections/rq-loss-function.tex <==
% !TEX root = ../main.tex
\subsection{\RQ{4}: The performance of the models with different pruning goals}

% TODO: Double-check average numbers and results compared to the files saved on the disk
\begin{table}
\centering
\caption{Comparison of the models on the NJR-1, XCorpus, and YCorpus datasets with three different pruning goals}
\label{tab:pruning-goals}
\vspace{-6pt}
\footnotesize
\input{tables/comparison-pruning-goals}
\end{table}

In our evaluation, the three datasets are imbalanced, especially NJR-1, as can be seen from the P/R ratio in Table~\ref{tab:data-stats}. This implies that there are substantially more false edges that need to be pruned compared to the number of true edges. Therefore, if both true and false edges are treated equally in the training phase, the ML models will likely be biased toward false edges. Motivated by this, we introduce three pruning goals: aggressive, conservative, and balanced. 

\paragraph{Methodology} We train and evaluated ML-based call graph pruners with three different pruning goals, namely, \textit{conservative}, \textit{aggressive}, and \textit{balanced}. Each goal assigns a different weight to prune/retain edges in the cross entropy loss function (see equation ~\ref{eq:cross-entropy}). They are explained as follows:

\begin{description}
%
\item[Conservative] Prioritizes high recall by maintaining as many edges as possible and only prunes when certain. Models are trained with 0.80 weight for keeping edges and 0.20 for pruning, minimizing false negatives.
%
\item[Balanced] Strives for a precision-recall equilibrium. The goal is to prune many false edges (like aggressive) while preserving true ones (like conservative). Models are trained with equal weight, 0.50, for both pruning and keeping edges.
%
\item[Aggressive] Models prune more edges, ensuring higher precision at the cost of missing true positives. This strategy greatly shrinks call graphs size and minimizes false alarms in downstream analyses further. Models are trained with a 0.80 weight for pruning edges.
%
\end{description}

For RandomForest, we use \textit{class\_weight} parameter in Scikit-learn to implement the pruning strategies described above.

% \begin{itemize}
%     \item \textit{Conservative}. The main goal here is to maintain a high recall. This means that the model aims to keep as many edges as possible, similar to WALA's original call graph, while detecting false edges when it is sure. This should also result in fewer false negatives (i.e., fewer edges incorrectly identified as unnecessary). The models are trained with 0.80 weight for keeping edges and 0.20 for pruning them. In other words, the models will be penalized more if pruning true edges.

%     \item \textit{Aggressive}. With this strategy, the models tend to prune more edges while maintaining a reasonable recall. Hence, the pruned call graphs have much higher precision while losing edges that were actually necessary (true positives). The aggressive strategy is useful to greatly reduce the size of the call graphs and prioritize much fewer false alarms in client analyses. To train the models for this goal, 0.80 weight is given for pruning edges. Therefore, the models will be rewarded when pruning false edges.

%     \item \textit{Balanced}. As the name suggests, this strategy seeks to strike a balance between precision and recall by optimizing for both. The goal is to remove as many false edges as possible (like the aggressive strategy) while also trying to keep as many true edges as possible (like the conservative strategy). This strategy is more suitable for applications where higher precision is demanded but losing edges might be costly. To train the models for this strategy, we give equal weight, i.e., 0.50 to both pruning and keeping edges.
% \end{itemize}

\paragraph{Results} \todo{The ratio of size(table) to size(explaining text) is not acceptable... expand on what the table contains, to which numbers you are referring etc... the table in itself is useless if not explained well. So either expand the text or cut the table (e.g., to just F1 values, or make clear that you are only referring to the averages). Why do we even have so many models in there? Why not Just the best one, then the table has only three rows: conservative, balanced, and aggressive}
Table~\ref{tab:pruning-goals} shows the performance of the models on the NJR-1, XCorpus, and YCorpus datasets considering three pruning goals, i.e., Conservative, Balanced, and Aggressive. Here, our first observation is that the conservative pruning goal gives a higher F1 score compared to the other two pruning goals across all three datasets. For instance, considering the conservative goal, the F1-score of YCorpus is 49\% on average, which is 6\% and 14\% higher than that of balanced and aggressive goals, respectively. The second observation is that the balanced pruning goal is placed between the conservative and aggressive in terms of performance, which is expected. Its average F1 score is lower than that of the conservative goal and higher than that of the aggressive. Meanwhile, the aggressive goal gives the highest precision across all three datasets which comes at the expense of much lower recall. For instance, Considering YCorpus, the average precision score of aggressive is 20\% higher than that of the conservative.
%  It provides a relatively acceptable \todo{?!?! what does "relatively acceptable" mean? Avoid such inconcrete formulations in a paper at all cost.} level of precision and recall.

Another important observation is that the F1-score of CGPruner's pruned call graphs is significantly improved in all three datasets if the conservative pruning goal is considered. For example, CGPruner's F1-score is 59\% on YCorpus with the conservative goal, which is 22\% higher than the same model and dataset with no pruning goal.

\todo{Just pointing out the obvious, but for our claimed "best dataset", the previous approaches outperform the LMs for conservative and balanced... this must be pointed out as a result and put into context. Why is that? What does it mean?}

==> sections/rq-njr1.tex <==
% !TEX root = ../main.tex
\subsection{\RQ{2}: The performance of the models on the repaired NJR-1 dataset}


\begin{table*}
\centering
\caption{Comparison of the ML-based call graph pruning models on the NJR-1 dataset and its repaired versions.}
\label{tab:njr1-vs-repaired}

\small
\vspace{-10pt}
(CGPruner does not use semantic features (de-compiled, recovered), so the results are the same for the three versions.)

\vspace{4pt}
\input{tables/comparison-njr-versions}
\end{table*}

\todo{at this point, it is not clear for me, why this is RQ1.1 and not a separate RQ?}
The original NJR-1 dataset only contains full source code for the target project and does not include the source code of its dependencies.
Prior work~\cite{le2022autopruner} introduced signature-based code feature for call graph nodes without source code (i.e., particularly for calls to dependencies) to alleviate this shortcoming.
The effect of this mix of representations and which representation is superior to the other is still unclear.
This motivated us to repair the dataset by recovering full source code for both source and target methods in call graphs and studying how this would affect the performance of the models at the call graph pruning task.

\paragraph{Methodology} We applied two strategies to augment the NJR-1 dataset with actual source code for the method bodies: de-compilation and original source code retrieval.

\begin{description}
%
\item[De-compilation] Utilizing Procyon~\cite{procyon}, an open-source Java de-compiler, we translated compiled class files into human-readable Java code. This method enables source code recovery without original source files, although the output may not exactly match the original, given that some information, such as comments and formatting, is lost during de-compilation.
%
\item[Repository-based Source Code Extraction] We identified dependencies in the NJR-1 dataset, located their respective repositories (often on platforms like GitHub), and directly downloaded the necessary source code. This approach preserves the original code, including comments, for deeper code understanding. However, it relies on the availability and accessibility of the repositories, which might not always be guaranteed.
%
\end{description}

We then extract semantic code features for both source code representations to fine-tune our code language models.
Our evaluation is limited to the 439K edges out of the total of 1.2M, for which we were able to acquire all three types of source code representation (signatures, decompiled, original source code).

\paragraph{Results}
Table~\ref{tab:njr1-vs-repaired} shows the performance of the ML models on the NJR-1 dataset and its repaired versions. Considering the F1 score, we observe that code language models perform very similarly on all the versions of NJR-1, namely, original, de-compiled, and recovered. The results obtained for RQ1.1 can be surprising as one would expect improvements in the pruned call graphs produced by the models trained and evaluated on the recovered version of NJR-1. It appears that code language models can still perform well even if the original dataset contains samples with a mix of both semantic and signature-based features. Moreover, it is interesting to see that, on average, all the code language models perform slightly better on the de-compiled version than the recovered version. This implies that the de-compilation method can be considered a viable alternative to the source code recovery in repairing the NJR-1 dataset.



==> sections/rq-overhead.tex <==
% !TEX root = ../main.tex
\subsection{\RQ{5}: The computational cost of different code features and the models' inference}

In general, call graph pruning is an extra step that is performed on static call graphs to prune false edges. This step involves both feature extraction and model inference, which adds additional overhead to static call graph construction. In this RQ, specifically, we show the computational cost of the code representations (described in subsection~\ref{sec:feat}) and doing pruning using the ML models, described in subsection~\ref{sec:models}).

\paragraph{Methodology} We measure the computation time for code features, namely, the structural~($f_{struct}$), signature~($f_{sig}$), semantic~($f_{sem}$), combined~($f_{comb}$), and call site-based~($f_{cs}$) features.
\todo{Unclear, how do you measure a feature? Are you measuring the extraction of the resulting speed of the model?}
Specifically, we iterate over 41 test programs in the NJR-1 dataset and report the average extraction time for these code features.

In the second experiment, we measure inference time 
\todo{shouldn't we call it "pruning time"? Why "inference"?}
for the ML-based call graph pruners, i.e., CGPruner~\cite{utture2022striking}, AutoPruner~\cite{le2022autopruner}, CodeBERT, CodeT5, and CodeT5+. Similarly, we iterate over all test programs in the NJR-1 dataset and report the average inference time per test program. Also, we report the size of the trained models on the disk. For the two experiments, we used only the NJR-1 dataset as it has more test programs. Besides, the extraction/inference time for both code features and models is correlated with their computational complexity regardless of the dataset size or choice.

\paragraph{Results} Table~\ref{tab:feat-ext-time} shows the extraction time for the five different code representations for the call graph pruning task. The signature-based feature, $f_{sig}$ is quickest, i.e., 1.5 seconds on average per test program, as it contains much fewer tokens compared to $f_{sem}$ when tokenizing. Also, both $f_{struct}$ and $f_{sem}$ have 5.02 seconds and 5.91 seconds, respectively. For $f_{sem}$, the extraction time is sensitive to the number of tokens in the dataset while, for $f_{struct}$, the number of nodes/edges in call graphs affect the extraction time. The call site-based representation, $f_{cs}$, takes 6.21 seconds on average per test program, which is slightly higher than that of $f_{sig}$.
This is expected as $f_{cs}$ needs to locate call sites in the source method and remove all other statements.
\revise{The overhead comes on top of the time it takes to generate a CG.
As the average CG generation with WALA takes about \checkNum{139s}, it can be concluded that the overhead of all approaches is small compared to the CG generation.}

Table~\ref{tab:inf-time-models} shows the inference time and size for the ML models studied in this paper. We also reported the time it takes to construct static call graphs using WALA. This would give a better idea of the additional computational cost introduced by the ML-based call graph pruners. CGPruner~\cite{utture2022striking} is the fastest and smallest model, with less than 0.1 seconds inference time, among the other models as it uses RandomForest as a classifier. Code language models like AutoPruner and CodeT5 do inference in 26 and 30 seconds, respectively. This is significantly higher than a RandomForest model as they are based on complex deep neural networks, namely, Transformers~\cite{vaswani2017attention}, with many learnable parameters. Also, the size of these code language models is around ~1.4GB, i.e., more than 4 times larger than RandomForest.

\begin{table}
\centering
\caption{Computational cost of different code features}
\label{tab:feat-ext-time}
\vspace{-6pt}
\small
\input{tables/computational-cost}
%\end{table}
\vspace{12pt}
%\begin{table}
\centering
\caption{Inference time and size for the models}
\label{tab:inf-time-models}
\vspace{-6pt}
\small
\input{tables/inference-time}
\end{table}

\todo{Major point: At the end of the experiments you have shown in various ways that CGs get smaller and that the pruning is fast... at no point does the paper show an actual advantage of prunign though. Why would someone want to prune their CGs? What happened to our client analyses?}




==> sections/summary.tex <==
% !TEX root = ../main.tex
\section{Summary}
\label{sec:summary}

\todo{shorten to about 1/3 of a text column}
In this paper, we conducted an empirical study on the effectiveness of machine learning-based call graph pruning. To this end, we identified three issues in the current state of research on ML-based call graph pruning: (1) the lack of a dataset with high test coverage for training and evaluation, (2) The effect of using source and target methods' signatures to compensate for lack of source code was unclear, (3) The ML models were trained on an imbalanced dataset without considerations in the learning phase. To study and address these three issues, we added the XCorpus to the evaluation and created a new dataset, YCorpus, with an average test coverage of 88\%. We also attempted to repair the NJR-1 dataset by recovering the complete source code and using a Java decompiler. To combat the third issue, we introduced three pruning goals, conservative, balanced, and aggressive. Our empirical results, based on three datasets, show that ML-based call graph pruning is promising and substantially improves the precision of call graphs. Second, both de-compilation and full source code recovery did not improve the pruned call graphs by the models compared to the original NJR-1 dataset, which is unexpected. Third, both conservative and balanced pruning goals improve the performance of the models further compared to the models with no pruning goal. Fourth, among the studied five code features for the call graph pruning task, our call site-based representation was shown to be as effective as the semantic feature and even better in some cases, such as CodeT5+ and NJR1. Finally, we showed that ML-based call graph pruning is computationally cheaper than static call graph construction. Hence, it is practical to be used outside a research environment.

% For future research, we will create a larger benchmark dataset than YCorpus, which has more Java projects and very high test coverage, >85\%. In addition, it would be interesting to investigate whether ML models can complement static call graphs by adding edges. 


==> tables/comparison-all-datasets.tex <==
\begin{tabular}{@{}lccccccccc@{}}
\toprule
& \multicolumn{3}{c}{\textbf{NJR-1}} & \multicolumn{3}{c}{\textbf{XCorpus}} & \multicolumn{3}{c}{\textbf{YCorpus}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
{\bf Models} & P & R & F1 & P & R & F1 & P & R & F1 \\
\midrule
\textbf{CGPruner} &  \textbf{0.72} & 0.53 & 0.53 & 0.50 & 0.29 & 0.35 & \textbf{0.72} & 0.25 & 0.37 \\
\textbf{AutoPruner} & 0.63 & 0.70 & 0.63 & 0.54 & 0.43 & 0.43 & 0.53 & \textbf{0.54} & \textbf{0.47} \\
\textbf{CodeBert} & 0.63 & 0.71 & 0.64 & 0.55 & \textbf{0.44} & \textbf{0.43} & 0.53 & 0.51 & \textbf{0.47} \\
\textbf{CodeT5} & 0.66 & 0.72 & 0.65 & 0.58 & 0.40 & 0.39 & 0.53 & 0.50 & 0.43 \\
\textbf{CodeT5+} & 0.64 & \textbf{0.76} & \textbf{0.66} & \textbf{0.61} & 0.24 & 0.26 & 0.58 & 0.49 & 0.44 \\
\midrule
\textbf{Average} & 0.65 & 0.68 & 0.62 & 0.56 & 0.36 & 0.37 & 0.58 & 0.46 & 0.44 \\
\midrule
\textbf{Wala} & 0.24 & 0.95 & 0.34 & 0.39 & 0.95 & 0.47 & 0.22 & 0.89 & 0.34 \\
\bottomrule
\end{tabular}

==> tables/comparison-code-features.tex <==
\begin{tabular}{@{}llcccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Code Features}} & \multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{NJR-1}} & \multicolumn{3}{c}{\textbf{XCorpus}} & \multicolumn{3}{c}{\textbf{YCorpus}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
& & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
\midrule
\multirow{1}{*}{$f\_{struct}$} & \textbf{CGPruner~\cite{utture2022striking}} & \textbf{0.72} & 0.53 & 0.53 & 0.50 & 0.29 & 0.35 & \textbf{0.72} & 0.25 & 0.37 \\
\midrule
\multirow{3}{*}{$f\_{sem}$} 
& \textbf{CodeBert} & 0.63 & 0.71 & 0.64 & 0.55 & 0.44 & 0.43 & 0.53 & 0.51 & 0.47 \\
& \textbf{CodeT5} & 0.66 & 0.72 & 0.65 & 0.58 & 0.40 & 0.39 & 0.53 & 0.50 & 0.43 \\
& \textbf{CodeT5+} & 0.64 & 0.76 & 0.66 & 0.61 & 0.24 & 0.26 & 0.58 & 0.49 & 0.44 \\
\midrule
\multirow{3}{*}{$f\_{sig}$} 
% & \textbf{AutoPruner~\cite{le2022autopruner}} & 0.63 & 0.69 & 0.63 & - & - & - &  - & - & - \\
& \textbf{CodeBert} & 0.62 & 0.61 & 0.57 & 0.51 & 0.44 & 0.43 & 0.64 & 0.54 & 0.48 \\
& \textbf{CodeT5} & 0.63 & 0.67 & 0.61 & 0.56 & 0.31 & 0.34 & 0.67 & \textbf{0.55} & \textbf{0.51} \\
& \textbf{CodeT5+} & 0.61 & 0.71 & 0.61 & 0.57 & 0.27 & 0.27 & 0.68 & 0.54 & 0.49 \\
\midrule
\multirow{3}{*}{$f\_{comb}$} 
& \textbf{AutoPruner~\cite{le2022autopruner}} & 0.63 & 0.70 & 0.63 & 0.54 & 0.43 & 0.43 &  0.53 & 0.54 & 0.47 \\
% & \textbf{CodeBert} & 0.63 & 0.70 & 0.63 & - & - & - & - & - & - \\
& \textbf{CodeT5} & 0.66 & 0.72 & 0.65 & 0.54 & 0.42 & 0.43 & 0.55 & 0.50 & 0.44 \\
& \textbf{CodeT5+} & 0.64 & \textbf{0.77} & 0.67 & 0.60 & 0.34 & 0.37 & 0.61 & 0.50 & 0.44 \\
\midrule
\multirow{3}{*}{$f\_{cs}$} 
% & \textbf{AutoPruner~\cite{le2022autopruner}} & 0.63 & 0.69 & 0.63 & - & - & - &  - & - & - \\
& \textbf{CodeBert} & 0.62 & 0.71 & 0.63 & 0.53 & \textbf{0.45} & \textbf{0.44} & 0.53 & 0.54 & 0.47 \\
& \textbf{CodeT5} & 0.65 & 0.72 & 0.65 & 0.55 & 0.31 & 0.34 & 0.54 & 0.50 & 0.43 \\
& \textbf{CodeT5+} & 0.66 & \textbf{0.77} & \textbf{0.68} & \textbf{0.62} & 0.24 & 0.24 & 0.59 & 0.47 & 0.43 \\
\midrule
 & \textbf{Wala} & 0.24 & 0.95 & 0.34 & 0.39 & 0.95 & 0.47 & 0.22 & 0.89 & 0.34 \\
\bottomrule
\end{tabular}


==> tables/comparison-njr-versions.tex <==
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
& \multicolumn{3}{c}{\textbf{Original}} & \multicolumn{3}{c}{\textbf{De-compiled}} & \multicolumn{3}{c}{\textbf{Recovered}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
{\bf Models} & P & R & F1 & P & R & F1 & P & R & F1 \\
\midrule
\textbf{CGPruner~\cite{utture2022striking}}\tnote{1} & 0.61 & 0.48 & 0.47 & 0.61 & 0.48 & 0.47 & 0.61 & 0.48 & 0.47  \\
\textbf{AutoPruner~\cite{le2022autopruner}} & 0.60 & 0.67 & 0.59 & 0.60 & 0.63 & 0.57 & 0.58 & 0.63  & 0.57 \\
\textbf{CodeBERT} & 0.61 & 0.66 & 0.59 & 0.60 & 0.65 & 0.57 & 0.59 & 0.61 & 0.56 \\
\textbf{CodeT5} & \textbf{0.63} & 0.66 & 0.60 & \textbf{0.64} & 0.69 & 0.62 & \textbf{0.63} & 0.64 & 0.60 \\
\textbf{CodeT5+} & 0.62 & \textbf{0.76} & \textbf{0.64} & 0.63 & \textbf{0.76} & \textbf{0.65} & \textbf{0.63} & \textbf{0.73} &  \textbf{0.64} \\
\midrule
\textbf{Average} & 0.61 & 0.65 & 0.58 & 0.62 & 0.64 & 0.58 & 0.61 & 0.62 & 0.57 \\
\midrule
\textbf{Wala} & 0.26 & 0.96 & 0.35 & 0.26 & 0.96 & 0.35 & 0.26 & 0.96 & 0.35 \\
\bottomrule
\end{tabular}

==> tables/comparison-pruning-goals.tex <==
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{NJR-1}} & \multicolumn{3}{c}{\textbf{XCorpus}} & \multicolumn{3}{c}{\textbf{YCorpus}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
\midrule
\multicolumn{10}{c}{Conservative} \\
\midrule
\textbf{CGPruner} & 0.62 & 0.64 & 0.59 & 0.44 & 0.63 & 0.49 & 0.59 & 0.64 & \textbf{0.59} \\
\textbf{AutoPruner} & 0.56 & 0.83 & 0.64 & 0.49 & \textbf{0.69} & \textbf{0.51} & 0.43 & \textbf{0.69} & 0.50  \\
\textbf{CodeBert} & 0.55 & 0.83 & 0.63 & 0.49 & 0.63 & 0.50 & 0.46 & 0.65 & 0.48 \\
\textbf{CodeT5} & \textbf{0.57} & 0.85 & \textbf{0.66} & 0.49 & 0.60 & 0.45 & 0.48 & 0.60 & 0.45 \\
\textbf{CodeT5+} & 0.55 & \textbf{0.89} & 0.65 & \textbf{0.55} & 0.33 & 0.34 & \textbf{0.49} & 0.58 & 0.45 \\
\midrule
\textbf{Average} & 0.57 & 0.81 & 0.63 & 0.49 & 0.58 & 0.46 & 0.49 & 0.63 & 0.49 \\
\midrule
\multicolumn{10}{c}{Balanced} \\
\midrule
\textbf{CGPruner} & \textbf{0.72} & 0.54 & 0.53 & 0.50 & 0.29 & 0.35 & \textbf{0.72} & 0.25 & 0.37 \\
\textbf{AutoPruner} & 0.63 & 0.70 & 0.63 & 0.52 & 0.40 & 0.40 & 0.52 & \textbf{0.56} & \textbf{0.49}   \\
\textbf{CodeBert} & 0.63 & 0.71 & 0.63 & 0.53 & \textbf{0.45} & \textbf{0.44} & 0.54 & 0.48 & 0.45 \\
\textbf{CodeT5} & 0.65 & 0.73 & 0.65 & 0.55 & 0.31 & 0.34 & 0.57 & 0.50 & 0.44 \\
\textbf{CodeT5+} & 0.65 & \textbf{0.76} & \textbf{0.67} & \textbf{0.61} & 0.25 & 0.25 & 0.57 & 0.49 & 0.45 \\
\midrule
\textbf{Average} & 0.66 & 0.69 & 0.62 & 0.54 & 0.36 & 0.36 & 0.58 & 0.46 & 0.44 \\
\midrule
\multicolumn{10}{c}{Aggressive} \\
\midrule
\textbf{CGPruner} & 0.69 & 0.40 & 0.44 & 0.47 & 0.23 & 0.28 & 0.67 & 0.27 & 0.36 \\
\textbf{AutoPruner} & 0.70 & 0.52 & 0.57 & \textbf{0.59} & 0.19 & 0.26 & \textbf{0.70} & 0.25 & 0.33  \\
\textbf{CodeBert} & 0.71 & 0.43 & 0.50 & 0.55 & \textbf{0.32} & \textbf{0.38} & 0.69 & \textbf{0.30} & \textbf{0.36} \\
\textbf{CodeT5} & 0.74 & 0.49 & 0.55 & 0.62 & 0.18 & 0.25 & 0.70 & \textbf{0.30} & 0.35 \\
\textbf{CodeT5+} & \textbf{0.73} & \textbf{0.60} & \textbf{0.62} & 0.65 & 0.16 & 0.19 & 0.70 & 0.27 & 0.34 \\
\midrule
\textbf{Average} & 0.71 & 0.49 & 0.53 & 0.58 & 0.22 & 0.27 & 0.69 & 0.28 & 0.35 \\
\midrule
\textbf{Wala} & 0.24 & 0.95 & 0.34 & 0.39 & 0.95 & 0.47 & 0.22 & 0.89 & 0.34 \\
\bottomrule
\end{tabular}


==> tables/computational-cost.tex <==
\begin{tabular}{@{}lrr@{}}
\toprule
\multirow{2}{*}{\textbf{Features}} & \multicolumn{2}{c}{\textbf{Extraction Time [s]}} \\
\cmidrule{2-3}
 & Average & Std. Dev. \\ 
\midrule
$f_{struct}$ & 5.02 & $\pm$ 13.11 \\
$f_{sig}$ & 1.50 & $\pm$ 2.55 \\
$f_{sem}$ & 5.91 & $\pm$ 13.25 \\
$f_{comb}$ & 10.59 & $\pm$ 24.93  \\
$f_{cs}$ & 6.21 & $\pm$ 14.48  \\
\bottomrule
\end{tabular}

==> tables/inference-time.tex <==
\begin{tabular}{@{}lrrr@{}}
\toprule
 \multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{Model Size [GB]}} & \multicolumn{2}{c}{\textbf{Inference Time [s]}} \\
\cmidrule{3-4}
 &  & Average & Std. Dev. \\ 
\midrule
WALA & N/A & 139.1 & $\pm$ 250.8 \\
\midrule
CGPruner\cite{utture2022striking} & 0.3  & <0.1 & $\pm$ <0.1\\
AutoPruner\cite{le2022autopruner} & 1.4 & 26.0 & $\pm$ 60.6\\
CodeBERT & 1.4 & 27.1 & $\pm$ 60.5\\
CodeT5 & 1.3 & 29.9& $\pm$ 61.9 \\
CodeT5+ & 3.8 & 76.6 & $\pm$ 192.1\\
\bottomrule
\end{tabular}

==> tables/structural-features.tex <==
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Feature} & \textbf{Description} \\ \midrule
src-node-in-deg & number of edges ending in caller \\
src-node-out-deg & number of edges out of caller \\
dest-node-in-deg & number of edges ending in callee \\
dest-node-out-deg & number of edges out of callee \\
depth & length of shortest path from main to caller \\
repeated-edges & number of edges from caller to callee \\
L-fanout & number of edges from the same call-site \\
node-count & number of nodes in call graph \\
edge-count & number of edges in call graph \\
avg-degree & average src-node-out-deg in call graph \\
avg-L-fanout & average L-fanout value in call graph \\
\bottomrule
\end{tabular}
